An EPTAS for Budgeted Matroid Independent Set

We consider the budgeted matroid independent set problem. The input is a ground set, where each element has a cost and a non-negative profit, along with a matroid over the elements and a budget. The goal is to select a subset of elements which maximizes the total profit subject to the matroid and budget constraints. Several well known special cases, where we have, e.g., a uniform matroid and a budget, or no matroid constraint (i.e., the classic knapsack problem), admit a fully polynomial-time approximation scheme (FPTAS). In contrast, already a slight generalization to the multi-budgeted matroid independent set problem has a PTAS but does not admit an efficient polynomial-time approximation scheme (EPTAS). This implies a PTAS for our problem, which is the best known result prior to this work. Our main contribution is an EPTAS for the budgeted matroid independent set problem. A key idea of the scheme is to find a representative set for the instance, whose cardinality depends solely on $1/\varepsilon$, where $\varepsilon > 0$ is the accuracy parameter of the scheme. The representative set is identified via matroid basis minimization, which can be solved by a simple greedy algorithm. Our scheme enumerates over subsets of the representative set and extends each subset using a linear program. The notion of representative sets may be useful in solving other variants of the budgeted matroid independent set problem.

==> guess.tex <==
%\section{Guessing Profitable elements}
%\label{sec:guess}

%In this section we describe the assignment of elements with relatively large profits 



\section{introduction}
\label{sec:introduction}

The problem of {\em budgeted matroid independent set (BMI)} consists of finding an independent set in a matroid with bounded {\em size} of maximal {\em profit}. TBA...


\includegraphics[scale=0.6]{1}

\section{Preliminaries}
\label{sec:preliminaries}

For the simplicity of the notations, for any set $A$ and some element $a$, let $A+a$, $A-a$ be $A \cup \{a\}$ and $A \setminus \{a\}$, respectively. In addition, for all $k \in \mathbb{N}$ let $[k] = \{1,2,\ldots,k\}$. Finally, for any function $f:A \rightarrow B$ and $C \subseteq A$ let $f(C) = \sum_{\ell \in C} f(\ell)$. 

\subsection{Matroids}

Let $E$ be a finite {\em ground set} and let $\cI \subseteq 2^E$ be a non-empty set containing subsets of $E$ called the {\em independent sets} of $E$. Then, $\cm = (E, \cI)$ is a {\em matroid} if the following holds: 

\begin{enumerate}
	\item (The Hereditary Property) For all $A \in \cI$ and $B \subseteq A$ it holds that $B \in \cI$.
	
	\item(The Exchange Property) For every $A,B \in \cI$ where $|A| > |B|$, there is $x \in A \setminus B$ such that $B +x \in \cI$. 
\end{enumerate}


A {\em basis} of a matroid $\cm = (E, \cI)$ is an independent set $B \in \cI$ such that for all $e \in E \setminus B$ it holds that $B+e \notin \cI$. Given a size function $s:E \rightarrow \mathbb{R}^{+}$, we say that a basis $B$ of $\cm$ is a {\em minimum} basis of $\cm$ w.r.t. $s$ if for any basis $A$ of $\cm$ it holds that $s(B) \leq s(A)$. A minimum basis w.r.t. $s$ of $\cm$ can be easily constructed in polynomial time using a greedy approach \cite{cormen2022introduction}. 

Throughout this paper, determining whether a subset of elements forms an independent set of a matroid is assumed to be relied on an {\em independence oracle}. Specifically, we assume that there is an oracle that given a matroid $\cm = (E, \cI)$ and a subset of elements $S \subseteq E$, returns "yes" if $S \in \cI$ and "no" otherwise. The next lemma gathers known results which follow from the definition of matroid (see, e.g., \cite{schrijver2003combinatorial} for more details). 

\begin{definition}
	\label{def:matroids}
Let $\cm = (E, \cI)$ be a matroid.  
	%
	\begin{enumerate}
		
		%\item For all $A,B \in \cI$ where $|A| \geq |B|$, there is $C \subseteq A \setminus B$, $|C| = |A|-|B|$ such that $B \cup C \in \cI$. 
		
		\item For every $F \subseteq E$ then define $\cm \cap F = (F, \cI')$ where $\cI' = \{A \in \cI~|~ A \subseteq F\}$. 
		
		%\item For every $F \subseteq E$ then $\cm - F = (E \setminus F, \cI')$ is a matroid where $\cI' = \{A \in \cI~|~ A \cap F = \emptyset\}$. 
		
		\item For every $F \in \cI$ then define $\cm / F = (E \setminus F, \cI')$ where $\cI' = \{A \subseteq E \setminus F~|~ A \cup F \in \cI\}$. 
		
		\item For every $q \in \mathbb{N}$ then define $[\cm]_{\leq q} = (E, \cI_{\leq q})$ where $\cI_{\leq q} = \{A \in \cI~|~ |A| \leq q\}$. 
		
	\end{enumerate}
\end{definition}

\begin{lemma}
	\label{lem:prel}
	
	The following conditions hold for any matroid $\cm = (E, \cI)$. 
	%
	\begin{enumerate}
		
		\item For all $A,B \in \cI$, there is $C \subseteq A \setminus B$, $|C| = \max\{|A|-|B|,0\}$ such that $B \cup C \in \cI$. 
		
			\item For every $F \subseteq E$ then $\cm \cap F$ is a matroid. 
		
		%\item For every $F \subseteq E$ then $\cm - F = (E \setminus F, \cI')$ is a matroid where $\cI' = \{A \in \cI~|~ A \cap F = \emptyset\}$. 
		
		\item For every $F \in \cI$ then $\cm / F$ is a matroid. 
		
		\item For every $q \in \mathbb{N}$ then $[\cm]_{\leq q} $ is a matroid.
	\end{enumerate}
	\comment{
	\begin{enumerate}
		
		\item For all $A,B \in \cI$ where $|A| \geq |B|$, there is $C \subseteq A \setminus B$, $|C| = |A|-|B|$ such that $B \cup C \in \cI$. 
		
			\item For every $F \subseteq E$ then $\cm | F = (F, \cI')$ is a matroid where $\cI' = \{A \in \cI~|~ A \subseteq F\}$.  (restriction)
		
		\item For every $F \subseteq E$ then $M - F = (E', \cI')$ is a matroid called the deletion of $F$ in $M$ where $E' = E \setminus F$ and $\cI' = \{A \in \cI~|~ A \cap F = \emptyset\}$. 
		
		\item For every $F \in \cI$ then $M / F = (E', \cI')$ is a matroid called the contraction of $F$ in $M$ where $E' = E \setminus F$ and $\cI' = \{A \subseteq E'~|~ A \cup F \in \cI\}$. 
		
			\item For every $q \in \mathbb{N}$ then $M^q = (E, \cI^q)$ is a matroid called the truncation of $q$ in $M$ where $\cI^q = \{A \in \cI~|~ |A| \leq q\}$. 
	\end{enumerate}
}
	\end{lemma}


\subsection{Matroid polytope}

%with $n$ elements numbered as $\{1,\ldots,n\}$
%A {\em basis} of $M$ is an independent set $B \in \cI$ such that for all $a \in E \setminus B$ it holds that $B+a \notin \cI$. Let $\textsf{bases}(M)$ be the set of all bases of $M$. Given a basis $B$ of $M$, 

Let $\cm = (E, \cI)$ be a matroid. Given $B \in \cI$, the {\em indicator vector} of $B$ is the vector $\mathbbm{1}^B \in \{0,1\}^E$ where for all $i \in B$ and $j \in [n] \setminus B$ we have $\mathbbm{1}^B_i = 1$ and  $\mathbbm{1}^B_j = 0$, respectively. Then, the {\em matroid polytope} of $M$ is the convex hull of the set of indicator vectors of all independent sets of $\cm$: $P_{\cm} = \textsf{conv} \{\mathbbm{1}^B~|~B \in \cI\}$. Note that for any $\bar{x} \in P_{\cm}$ it holds that $\{e \in E~|~ \bar{x}_e \geq 1\} \in \cI$ (see, e.g., \cite{schrijver2003combinatorial}).%In addition, a {\em face} of a polytope $P$ is the intersection of P with any closed half-space whose boundary is disjoint from the interior of $P$. The next result is due to \cite{grandoni2010approximation}.
\comment{
 \begin{lemma}
	\label{lem:integral}
	Let $\cm$ be a matroid and let $F$ be a face of dimension
	$d$ of the matroid polytope $P_{\cm}$. Then any $\bar{x} \in F$ has at most $2d$ non-integral
	components.
\end{lemma}
}

\subsection{Instance and Solution}

%For all $Q \subseteq E$, let $s(Q) = \sum_{\ell \in Q} s(\ell)$ and $p(Q) = \sum_{\ell \in Q} p(\ell)$. 

Formally, a BMI instance is a tuple $\ck =  (E,\cI,s,p)$, where $(E,\cI)$ is a matroid, $s:E \rightarrow [0,1]$  gives the elements sizes, and $p:E \rightarrow \mathbb{R}^+$ gives the elements profits. A {\em solution} of $\ck$ is an independent set $X \in \cI$ such that $s(X) \leq 1$; in addition, the {\em profit} of the solution is $p(X)$ and let $\OPT(\ck)$ denote the profit of a solution of $\ck$ with maximal profit. As a subroutine of our scheme, we compute a constant factor approximation for BMI using the next result of  \cite{grandoni2010approximation}, applied with parameter $\eps' = \frac{1}{2}$. We denote by $|\ck|$ the encoding size of a BMI instance $\ck$.%In this section we prove the following result. 
 \begin{lemma}
	\label{lem:PTAS}
There is an algorithm \textnormal{\textsf{PTAS}} that given a \textnormal{BMI} instance $\ck$ and $0<\eps <\frac{1}{2}$, returns in time $|\ck|^{O(\frac{1}{\eps})}$ a solution of $\ck$ with profit at least $(1-\eps) \cdot \OPT(\ck)$.
\end{lemma}


\section{The Algorithm}
\label{sec:alg}


In this section we present our EPTAS for BMI. The algorithm handles elements with high profit separately; this is done by finding a small subset of {\em representatives}: elements from which the most profitable elements of the solution are selected. Additional elements with lower profits are then added using a {\em linear program (LP)}. For the remainder of this section, fix a BMI instance $\ck =  (E,\cI,s,p)$ and a parameter $0<\eps <\frac{1}{2}$, where without the loss of generality, we assume that $\eps^{-1} \in \mathbb{N}$ and that for all $\ell \in E$ we assume that $\{\ell\} \in \cI$ (otherwise $\ell$ cannot belong to any solution of $\ck$). %For the flow of the reading, some of the more technical proofs are deferred to Section~\ref{sec:proofs}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
In the following, we use rounding on profit of elements with relatively large profits. We start with computing a constant factor approximation of the optimum $\OPT(\ck)$. By the results of Grandoni and Zenklusen, the {\em $k$-budgeted matroid independent set} admits a PTAS \cite{grandoni2010approximation}. Since BMI is a special case of the latter problem with a single budget, using parameter $\eps' = \frac{1}{2}$, we can compute in polynomial time a solution $B^*$ of $\ck$ such that $p(B^*) \geq \frac{\OPT(\ck)}{2}$. Moreover, let $t = \eps^{-1}+1$ and let $h = \eps^t \cdot p(B^*)$. 

We say that an element $\ell \in E$ is {\em profitable} if $p(\ell) \geq h$ and {\em unprofitable} otherwise. Let $H$ denote the set of profitable elements; that is, $H = \{\ell \in E~|~ p(\ell) \geq h\}$. In our algorithm, we round the profits of the profitable elements down to the next multiple of $\eps \cdot h$; note that each elementmay lose only a small fraction of the profit by the above rounding (see Lemma~\ref{lem:J}). Formally, define the {\em profit classes} as $$T = \big\{r \cdot \eps \cdot h ~|~r \in \mathbb{N}_{>0}, r \cdot \eps \cdot h \leq 2 \cdot p(B^*)\big\}$$ which is the set containing the possible profits of profitable elements after the rounding. Now, define $\bar{p}: E \rightarrow \mathbb{R}^+$ as the {\em rounded profit function} such that for all unprofitable elements $\ell \in E \setminus H$ it holds that $\bar{p}(\ell) = p(\ell)$ and for all profitable elements $\ell \in H$ it holds that \begin{equation}
	\label{eq:max}
	\bar{p}(\ell) = \max_{\{y \in T~|~ y ~\leq ~ p(\ell)\}} y.
\end{equation} %Now, let $\cJ = (I,\mathcal{G},s,\bar{p},m,c)$ be the instance where the profits are rounded down as defined above. 


\begin{lemma}
	\label{lem:J}
	For any $A \subseteq E$ it holds that $\bar{p}(A) \geq (1-\eps) \cdot p(A)$. 
\end{lemma} 




Hence, by Lemma~\ref{lem:J} finding a solution with high profit w.r.t. $\bar{p}$ yields a solution with almost the same profit w.r.t. $p$; on the other hand, the number of distinct profits of profitable elements for $\bar{p}$ is bounded by a function of $\eps^{-1}$. Let $q = 2 \cdot \eps^{-t-1}$. By the next result, $q$ is an upper bound on the number of profitable elements in a solution of $\cm$ and on the number of profit classes. 


}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Let $t = \eps^{-1}+1$ and let $h = \eps^t \cdot \OPT(\ck)$. We say that an element $\ell \in E$ is {\em profitable} w.r.t. $\eps$  if $p(\ell) \geq h$ and {\em unprofitable} otherwise. 

In the following, we define the elements which are considered as {\em profitable} by our scheme. Let $t = \eps^{-1}+1$ and let $H = \{\ell \in E~|~ p(\ell) \geq \eps^t \cdot \OPT(\ck)\}$ be the set of {\em profitable} elements and let $E \setminus H$ be the set of {\em unprofitable} elements. Now, let $q(\eps) = \eps^{-t-1}$; our scheme constructs a subset of elements $R$ (representatives) of size bounded by $2 \cdot q^2(\eps)$ \ilan{update}. We enumerate over all subsets of the representative elements $F \subseteq R$, to determine the set of profitable elements returned by the scheme. Despite the small number of representative elements which depends solely on $\eps$, this simple approach loses only a small portion of the overall profit, in comparison to an optimal solution. \comment{By the next result, $q(\eps)$ is an upper bound on the number of profitable elements in a solution of $\ck$. 
\begin{lemma}
	\label{q}
	For any solution $A$ of $\ck$ it holds that $|H \cap A| \leq q(\eps)$. 
\end{lemma}}
%
%
%





The construction of the set of representative elements $R$ is explained below. First, we compute a $2$-approximation $S^{*}$ for $\ck$. Second, for each value $r \in [\log_{1-\eps} q(\eps)]$, we compute a minimum basis $B_r$ w.r.t. $s$ of the matroid imposed by the following restrictions on the matroid $(E,\cI)$: (i) the matroid is restricted only to elements $e \in E$ satisfying that $\frac{p(e)}{2 \cdot p(S^*)}$, i.e., the profit divided by an upper bound on $\OPT(\ck)$, belongs to the interval $\big( (1-\eps)^{r}, (1-\eps)^{r-1} \big]$; (ii) the independent sets of the matroid are restricted to contain at most $q(\eps)$ elements. Note that restricting $(E,\cI)$ with (i) and (ii) results in a matroid by Lemma~\ref{lem:prel}. Finally, the representative elements are defined as the union of the minimal bases $B_r$, for all $r \in [2 \cdot q(\eps)]$. 

The pseudocode of algorithm $\textsf{FindRep}$, which computes the set of representative elements in $E$, is given in Algorithm~\ref{alg:representative}. The next definition summarizes properties of the representative elements. \begin{definition}
	Given a \textnormal{BMI} instance $\ck = (E,\cI,s,p), 0<\eps<\frac{1}{2}$ and $R \subseteq E$, $R$ is a {\em representative set} of $\ck$, $\eps$ if for all $G \in \cI_{\leq q(\eps)} \cap 2^{H}$ there is $Z \in \cI_{\leq q(\eps)} \cap 2^R$ such that the following holds. \begin{enumerate}
		\item $s(Z) \leq s(G)$.
			\item $|Z|= |G|$. 
				\item $p(Z) \geq (1-\eps) \cdot p(G)$. 
					\item $\min_{e \in Z} p(e) \geq (1-\eps) \cdot \left( \min_{e \in G} p(e) \right)$. 
	\end{enumerate}
\end{definition}
%
%
%
%
%
 %For the next lemma, let $\cI^{q(\eps)} = \{A \in \cI~|~|A| \leq q(\eps)\}$. 
%
%
%
%For every profit class $y \in T$, let $E_y = \{\ell \in E~|~p(\ell) = y)\}$ be the subset of elements with profit $y$. For all $y \in T$, we construct a subset of elements $B_y \subseteq E_y$ independently of the remaining profit classes. Recall that the {\em truncation} of $q$ in $M$ is the matroid $M^q = (E,\cI^q)$ where $\cI^q = \{A \in \cI~|~ |A| \leq q\}$ contains all independent sets in $\cm$ with cardinality at most $q$. 
%
%We construct $B_y$ by taking the independent set in $E_y \cap \cI^q$ with maximal number of elements (i.e., a {\em basis}) that has a minimal total size of elements. This can be computed easily by the following greedy approach. Let $E_y  = \{y(1), \ldots, y(n_y)\}$ be non decreasing order of $E_y$ by element sizes; that is, for all $i,j \in [n_y], i \leq j$ we have $s\left(y(i)\right) \leq s\left(y(j)\right)$. Then, initialize $B_y = \emptyset$ and the next element$y(i) \in E_y$ according to the sorted order is added to $B_y$ if $B_y+y(i)$ forms an independent set in the truncation of $q$ in $M$. Finally, the representative elements are $S = \bigcup_{y \in T} B_y$ that is the union of the elements representative for $B_y$ for all profit classes. The algorithm for constructing the representative elements is reffered to as Algorithm \textsf{Chosen} and the pseudocode of the algorithm is given in Algorithm~\ref{alg:representative}. %\ilan{I dont have time in this iteration by I have a suggestion for improving Algorithm Chosen: to define a minimal basis with at most $q$ elementfor each $E_y$, and in the algorithm just write that we take the union of the minimal bases of all $y \in T$.}
%
%
%
 \begin{algorithm}[h]
	\caption{$\textsf{FindRep}(\ck = (E,\cI,s,p),\eps)$}
	\label{alg:representative}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	Compute a $2$-approximation $S^{*} = \textsf{PTAS}(\ck,\frac{1}{2})$ for $\ck$.
	
	%Initialize $R \leftarrow \emptyset$. 
		\For{$r\in [\log_{1-\eps} q(\eps)]$}{
		
		Compute a minimum basis $B_r$ w.r.t. $s$ of the matroid $\left[ (E, \cI) \cap \left\{e \in E~\bigg|~ \frac{ p(e)}{2 \cdot p(S^{*})} \in \big( (1-\eps)^{r}, (1-\eps)^{r-1} \big]\right\} \right]_{\leq q(\eps)}$.
		
		
	}
	\comment{
	\For{$r\in \left\{1,\ldots, \log_{1+\eps}\left(q(\eps)\right)\right\}$}{
		
	Compute a minimum basis $B_r$ w.r.t. $s$ of the matroid $\left((E, \cI) \bigoplus \left\{e \in E~\bigg|~p(e) \in \left[(1+\eps)^{r-1} \cdot  \eps^{t+1} \cdot p(S^{*}), (1+\eps)^r \cdot  \eps^{t+1} \cdot p(S^{*})\right]\right\}\right)^{q(\eps)}$ 
		
		
	}
}

Return $R = \bigcup_{r \in [\log_{1-\eps} q(\eps)]} B_r$.  

	%Return $R = \bigcup_{r \in  \left\{0,\ldots, \log_{1+\eps}\left(q(\eps)\right)\right\}} B_r$. 
\end{algorithm}
%
\comment{
 \begin{algorithm}[h]
	\caption{$\textsf{Chosen}((E,\cI,s,p),q,T)$}
	\label{alg:representative}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	\For{$y \in T$}{
		
		Initialize $B_y \leftarrow \emptyset$.
		
		Sort $E_y$ in non decreasing order by element ysizes $y(1), \ldots, y(n_y)$.\label{order}
		
		\For{$i = 1,\ldots,n_y$}{
			
			\If{$B_y + y(i) \in \cI^q$ \label{step:if}}{
				
				Update $B_y \leftarrow B_y+y(i)$
				
			} 
			
		}
		
	}
	
	Return $S = \bigcup_{y \in T} B_y$. 
\end{algorithm}
%
%
}
%
 %
 %
\begin{lemma}
	\label{lem:main}
	Given a \textnormal{BMI} instance $\ck = (E,\cI,s,p)$ and $0<\eps <\frac{1}{2}$, Algorithm~\ref{alg:representative} returns in time $O(|\ck|) \cdot O(q(\eps))$ a representative set $R$ of $\ck$ such that $|R| \leq  q(\eps) \cdot \log_{1-\eps} (q(\eps))$. \comment{such that the following holds. \begin{itemize}
		\item . 
		%
		\item 	For all $G \in \cI^{q(\eps)} \cap 2^{H}$, there is $Z \in \cI^{q(\eps)} \cap 2^R$ such that (i) $s(Z) \leq s(G)$; (ii) $|Z|= |G|$; (iii) $p(Z) \geq (1-\eps) \cdot p(G)$; and (iv) $\min_{e \in Z} p(e) \geq (1-\eps) \cdot \left( \min_{e \in G} p(e) \right)$. 
		\comment{
		\begin{enumerate}
			\item$s(Z) \leq s(G)$.
			
			\item $|Z|= |G|$.
			
			\item $p(Z) \geq (1-\eps) \cdot p(G)$.
			
			\item $\min_{e \in Z} p(e) \geq (1-\eps) \cdot \left( \min_{e \in G} p(e) \right)$.
		\end{enumerate} 
	}
	\end{itemize}
	%
}
%
\end{lemma} The proof of Lemma~\ref{lem:main} is given in Section~\ref{sec:lemMainProof}. Lemma~\ref{lem:main} is the key component in the analysis of the scheme: the profitable elements of an optimal solution may be replaced by a subset of the representative elements with similar profit without increasing the total size of elements. However, for the unprofitable elements other techniques are required. 

We use an LP based on a matroid polytope to add unprofitable elements to the solution.  Let $F \subseteq E$ be some subset of elements. In the following, we define an LP whose objective is to find a subset of elements of maximal profit that together with $F$ forms a solution of $\ck$. Formally, let%Since $F$ may prevent an addition of an optimal subset of elements due to the matroid constraint, we use a relaxation which restricts the potential elements to be of significantly smaller profit in comparison with the elements in $F$. In the analysis, this turns out to be beneficial and decreases the potential profit only slightly by choosing an appropriate $F$. Formally, let 
\begin{equation}
	\label{E_F}
	E_F = \big\{\ell \in E~|~ p(\ell) \leq 2\eps \cdot \min_{j \in F} p(j)\big\}
\end{equation} be the {\em potential elements} for $F$; if $F = \emptyset$ then define $E_F = E$. The elements in $E_F$ are of profits bounded by $\eps$ times the minimal profit of an element in $F$. Now, define the $F$-{\em matroid} as $\cm_F = (E_F,\cI_F)$ where  $\cI_F = \{A \subseteq E_F~|~ A \cup F \in \cI\}$. Note that the $F$-matroid is indeed a matroid by properties $2,3$ of Lemma~\ref{lem:prel}. 

\begin{lemma}
	Let $\ck = (E,\cI,s,p)$ be a \textnormal{BMI} instance and let $0<\eps<\frac{1}{2}$. Also let R be a representatives set of K and $\eps$. Then, there is $Z\subseteq R$ and $T \subseteq E_Z$ such that the following holds.
	
	\begin{enumerate}
		%\item $Z\in \cI$
		\item $T \cup Z \in \cI$.
		\item $s\left(T\cup Z\right) \leq 1$.
		\item $p\left(T\cup Z\right) \geq (1-4\eps) \OPT(K)$.
	\end{enumerate} 
\end{lemma}

\begin{proof}
		Let $U$ be a solution of $\ck$ with profit $p(U) = \OPT(\ck)$. In the following, we partition a subset (with possibly empty sets in the partition) of the profitable elements in $U$ into $\eps^{-1}$ disjoint sets. Formally, for all $i \in \left[\eps^{-1}\right]$ let 
	%
	\begin{equation}
		\label{J_i}
		J_i = \big\{\ell \in H \cap U~\big|~ p(\ell) \in \big[\eps^{i+1} \cdot \OPT(\ck),  \eps^{i} \cdot \OPT(\ck) \big) \big\}		
	\end{equation}
	%
	%be all profitable elements in $U$ with profits in the interval $ \big[\eps^{i+1} \cdot \OPT(\ck),  \eps^{i} \cdot \OPT(\ck) \big) $. 
	%
	Since $J_1,\ldots, J_{\eps^{-1}}$ are $\eps^{-1}$ disjoint  subsets of elements within $U$, there is $i^* \in \left[\eps^{-1}\right]$ such that $p(J_{i^*}) \leq \eps \cdot \OPT(\ck)$ as otherwise it implies that $p(U) > \OPT(\ck)$ in contradiction. Now, define $J_0 = (H \cap U) \setminus \bigcup_{i \in [\eps^{-1}]} J_i$ as the set containing the largest profitable elements in $H \cap U$ not counted in the above subsets; in addition, let $L =  \bigcup_{k < i^*} J_k$ (including $J_0$) be the {\em most profitable} elements and let $Q = U \setminus (L \cup J_{i^*})$ be the {\em less profitable} elements. We now show that $L \in \cI^{q(\eps)}$. 
	%
		%Thus, to show that $L \in \cI^{q(\eps)}$, we show that $|L| \leq q(\eps)$.  %in addition, since $q(\eps) = \eps^{-t-1}$ and $p(\ell) \geq \eps ^{t} \cdot \OPT ~\forall \ell \in H \cap U$, it holds that $|L| \leq q(\eps)$ or $p(L) > \OPT(\ck)$ in contradiction that $L$ is a solution of $\ck$. Hence, $L \in \cI^{q(\eps)}$
	%
	\begin{equation}
		\label{contradiction1}
		\begin{aligned}
			p(U) ={} & \sum_{\ell \in U} p(\ell) \geq  \sum_{\ell \in H \cap U} p(\ell) \geq \sum_{\ell \in L}  \eps^{t} \cdot \OPT(\ck)  = \eps^{t} \cdot \OPT(\ck) \cdot |L|.
		\end{aligned}
	\end{equation} The second inequality is because for all $\ell \in H$ it holds that $p(\ell) \geq  \eps^{t} \cdot \OPT(\ck)$. Since $L \subseteq H \cap U$, by the hereditary property of $(E,\cI)$ it holds that $L \in \cI$. Thus, by \eqref{contradiction1} it follows that $L \in \cI_{\leq q(\eps)}$ (recall that $p(U) = \OPT(\ck)$ and $q(\eps) = \eps^{-t-1}$). 
%	\begin{claim}
	%	\label{claim:q}
	%	$L \in \cI^{q(\eps)}$. 
	%\end{claim}
	%Since $L \subseteq H \cap U$, by the hereditary property it holds that $L \in \cI$; in addition, since $q(\eps) = \eps^{-t-1}$ and $p(\ell) \geq \eps ^{t} \cdot \OPT ~\forall \ell \in H \cap U$, it holds that $|L| \leq q(\eps)$ or $p(L) > \OPT(\ck)$ in contradiction that $L$ is a solution of $\ck$. Hence, $L \in \cI^{q(\eps)}$; then, 
	Because $L \in \cI_{\leq q(\eps)}$, the conditions of Theorem~\ref{lem:main} are satisfied for $L$; hence, there is $Z \subseteq R$ such that $Z \in \cI_{\leq q(\eps)}$, $s(Z) \leq s(L)$, $|Z| = |L|$, $p(Z) \geq (1-\eps) \cdot p(L)$, and $\min_{e \in Z} p(e) \geq (1-\eps) \cdot \left( \min_{e \in G} p(e) \right)$.  %Then, because $Z \subseteq R$, there is an iteration of Algorithm~\ref{alg:EPTAS} such that $F = Z$ in Step~\ref{step:for}. We define a point in $\textnormal{LP}(\ck,Z)$ whose definition is relied on the following subset of elements. First, if $|Z| > |Q|$ then define $C = \emptyset$. Otherwise, $|Q| \geq |Z|$; then, by Lemma~\ref{lem:prel} there is $C' \subseteq Q \setminus Z, |C'|  = |Q| - |Z|$ such that $Z \cup C' \in \cI$; in this case, define $C = C'$. Now, define $\bar{x}^* \in \{0,1\}^{E_Z}$ such that for all $\ell \in C$ define $\bar{x}^*_{\ell} = 1$ and for all $\ell \in E_Z \setminus C$ define $\bar{x}^*_{\ell} = 0$. 
	
	Because $U \in \cI$ and $Q \subseteq U$, by the hereditary property it follows that $Q \in \cI$. Therefore, by Lemma~\ref{lem:prel} there is $T \subseteq Q \setminus Z, |T|  = \max\{|Q| - |Z|,0\}$ such that $Z \cup T \in \cI$. Observe that 
	%
	\begin{equation}
		\label{EZZ}
		\begin{aligned}
				T \subseteq{} & Q \subseteq \{e \in E~|~p(e) \leq \eps^{i^*+1} \cdot \OPT(\ck)\} =  \{e \in E~|~p(e) \leq \eps \cdot \eps^{i^*} \cdot \OPT(\ck)\} \\  \subseteq{} &  \{e \in E~|~p(e) \leq \eps \cdot \min_{e \in L} p(e)\} \subseteq  \{e \in E~|~p(e) \leq \frac{\eps}{1-\eps} \cdot \min_{e \in Z} p(e)\} \subseteq E_Z.
		\end{aligned}
	\end{equation} The second and third inclusions are by \eqref{J_i}. The fourth inclusion is because $\min_{e \in Z} p(e) \geq (1-\eps) \cdot \left( \min_{e \in G} p(e) \right)$. The last inclusion is because $0<\eps <\frac{1}{2}$ and by \eqref{E_F}. By \eqref{EZZ} it follows that $T \subseteq E_Z$.To conclude the proof, we show the last two properties of the lemma. 
	%
	%
	%
	%Now, define $\bar{x}^* \in \{0,1\}^{E_Z}$ such that for all $\ell \in C$ define $\bar{x}^*_{\ell} = 1$ and for all $\ell \in E_Z \setminus C$ define $\bar{x}^*_{\ell} = 0$. 
		%
 $$ s(Z \cup T) = s(Z)+s(T) \leq s(L)+s(Q) \leq s(U) \leq 1.$$ The first inequality is because $s(Z) \leq s(L)$ and $T \subseteq Q$. The last inequality is because $U$ is a solution of $\ck$. We use the following inequality. 	\begin{equation}
 	\label{eq:men}
 	\begin{aligned}
 	p(Q \setminus T) \leq{} & |Q \setminus T| \cdot \max_{\ell \in Q \setminus T} p(\ell) \leq |Z| \cdot 2\eps \cdot  \min_{\ell \in Z} p(\ell) \leq 2\eps \cdot p(Z) \leq 2\eps \cdot \OPT(\ck).
 	\end{aligned}
 \end{equation} 
 
 \begin{equation*}
 	\begin{aligned}
 		p(Z \cup T) \geq{} & (1-\eps) \cdot p(L)+p(Q) - p(Q \setminus T) \leq (1-\eps) \cdot p(U) -2\eps \cdot \OPT(\ck) = (1-3\eps) \cdot  \OPT(\ck).
 	\end{aligned}
 \end{equation*} 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 \comment{ 
 
 The last inequality is by Lemma~\ref{lem:main}. By the above and by \eqref{LP}, it holds that $\bar{x}^*$ satisfies the conditions of $\textnormal{LP}(\ck,Z)$. To conclude the proof, we use the following inequalities. If $L \neq \emptyset$ the following holds:
	%
	\begin{equation}
		\label{eq:11}
		\begin{aligned}
			\eps \cdot p(Z)-p(Q \setminus C) \geq{} & 	\eps \cdot p(Z)-|Q \setminus C| \cdot \max_{\ell \in Q \setminus C} p(\ell) \geq \eps \cdot p(Z)- |Z| \cdot \eps \cdot  \min_{\ell \in L} p(\ell) \\ \geq{} & \eps \cdot p(Z)- |Z| \cdot   \frac{\eps \cdot \min_{\ell \in Z} p(\ell)}{(1-\eps)} \geq \eps \cdot p(Z)-2\eps \cdot p(Z) \geq -\eps \cdot \OPT(\ck).
		\end{aligned}
	\end{equation} The second inequality is because $C \subseteq Q \setminus Z$, $|C|  = |Q| - |Z|$ or $C = \emptyset$ if $|Z| > |Q|$ and it follows that $|Q \setminus C| \leq |Z|$; in addition, by \eqref{J_i} and the definition of $L,Q$ it holds that all elements in $Q \setminus C$ are of profits at most $\eps \cdot \min_{\ell \in L} p(\ell)$ for $L \neq \emptyset$. The third inequality is by Lemma~\ref{lem:main}. The fourth inequality is because $0<\eps <\frac{1}{2}$. The last inequality is because $p(Z) \leq \OPT(\ck)$, since $Z$ is a solution of $\ck$ because $L$ is a solution of $\ck$ and by Lemma~\ref{lem:main}. Furthermore, 
	%
	\begin{equation}
		\label{eq:p(x)2}
		\begin{aligned}
			p(Z)+p(Q) \geq{} & (1-\eps) \cdot p(L)+ p(Q) \geq  (1-\eps) \left( p(L)+p(Q)\right) =  (1-\eps)  p(U \setminus J_{i^*}) \\ \geq{} & (1-\eps) (1-\eps)\OPT(\ck) \geq (1-2\eps)  \OPT(\ck). 
		\end{aligned}
	\end{equation} The first inequality is by Lemma~\ref{lem:main}. The third inequality is because $p(J_{i^*}) \leq \eps \cdot \OPT(\ck)$. Therefore,%The first equality is because $Z,L \subseteq H$ and for all $y \in T$ it holds that $|Z \cap E_y| = |E_y \cap L|$. The second inequality is by Lemma~\ref{lem:J}. Therefore,
	%
	\begin{equation*}
		\label{eq:p(x)}
		\begin{aligned}
			p(Z)+\sum_{\ell \in E_Z} \bar{x}^*_{\ell} \cdot p(\ell) ={} & p(Z)+\sum_{\ell \in C} p(\ell) = p(Z)+p(C) = p(Z)+p(Q) - p(Q \setminus C) \\ \geq{} & (1-\eps) (p(Z)+p(Q))+\eps \cdot p(Z)-p(Q \setminus C)  \geq (1-4\eps) \OPT(\ck).
		\end{aligned}
	\end{equation*} The last inequality is by \eqref{eq:11} and \eqref{eq:p(x)2}.  Hence, $\bar{x}^*$ satisfies the conditions of the claim. 

}
\end{proof}



Finally, define the following relaxation of the problem:
% In other words, the $F$-matroid is the deletion of $E\setminus E_F$ in $M$ combined with the contraction of $F$ in $\cm$; hence, 
 \begin{equation}
 	\label{LP}
 	\begin{aligned}
 		\textnormal{LP}(\ck,F)~~~~~~~~~~~~~~~~~ \max\quad        & ~~~\sum_{\ell \in E_F} \bar{x}_{\ell}   \cdot p(\ell)             ~~~~~~~~~~~~~~~~~~~~~                                                \\
 		\textsf{s.t.\quad} & ~~~\sum_{\ell \in E_F} \bar{x}_{\ell}  \cdot s(\ell)         \leq  1-s(F) ~~~~~~~~~~~~~~~~~~~~~           \\  
 		& ~~~\bar{x} \in P_{\cm_F} \\
 		%& ~~~\bar{x} \in [0,1]^{E_F} 
 	\end{aligned}
 \end{equation}  The linear program $\textnormal{LP}(\ck,F)$  maximizes the (fractional) total profit of a point in the $F$-matroid (i.e., $P_{\cm_F}$), with total size of elements at most $1-s(F)$; that is, the residual capacity of a solution without the elements in $F$. In particular, observe that there is no solution to the $\textnormal{LP}(\ck,F)$  if $s(F) > 1$ and there is only an all-zero solution in case that $F \notin \cI$. Since $F$ may prevent an addition of an optimal subset of elements due to the matroid constraint, the $\textnormal{LP}(\ck,F)$ restricts the potential elements of $F$ to be of significantly smaller profit in comparison with the elements in $F$, i.e., creating a {\em profit gap}. In the analysis, this turns out to be beneficial and decreases the potential profit only slightly by choosing an appropriate $F$.  The next lemma follows as a special case of a result of \cite{grandoni2010approximation}. \begin{lemma}
	\label{lem:integral}
		Let $\ck = (E,\cI,s,p)$ be a \textnormal{BMI} instance, $F \subseteq E$, and $\bar{x}$ be a basic solution to $\textnormal{LP}(\ck,F)$. Then, $\bar{x}$ has at most $2$ non-integral entries. 
\end{lemma}

%In addition, observe that a vertex $\bar{\lambda}$ of the $\textnormal{LP}(\ck,F)$  is in  a face of dimension $1$ (i.e., an edge) of the $F$-matroid polytope $P_{\cm_F}$, since the $\textnormal{LP}(\ck,F)$  is obtained from $P_{\cm_F}$ by adding a single linear constraint for bounding the capacity. Hence, by Lemma~\ref{lem:integral} it follows that $\bar{\lambda}$ has at most $2$ non-integral entries. 




 \begin{algorithm}[h]
	\caption{$\textsf{EPTAS}(\ck = (E,\cI,s,p),\eps)$}
	\label{alg:EPTAS}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	%Construct $q,T$ using a $2$-approximation for BMI. 
	
	Construct the representative elements $R = \textsf{FindRep}(\ck,\eps)$. 
	
	
	Initialize an empty solution $A \leftarrow \emptyset$.\label{step:init}
	
	\For{$F \subseteq R \text{ s.t. } F \in \cI$ \label{step:for}}{
		
		
		Find a basic optimal solution $\bar{\lambda}^F$ of the $\textnormal{LP}(\ck,F)$.\label{step:vertex}
		
		Let $C_F =  \{\ell \in E_F~|~ \bar{\lambda}^F_{\ell} \geq 1\} \cup F$.
		
			
			\If{$p\left(C_F\right) > p(A)$\label{step:iff}}{
				
				Update $A \leftarrow C_F$\label{step:update}
				
			} 
			
		
	}
	
	Return $A$. 
\end{algorithm}
%and round down the entries of $\bar{\lambda}^F$: let $\bar{\gamma}^F \in \{0,1\}^{E_F}$ be the vector where $\bar{\gamma}^F_{\ell} = \floor{\bar{\lambda}^F_{\ell}}$.  In addition, let
Using the above, we have the required components for designing the following EPTAS for BMI. Let $R$ be the representative elements returned by $\textsf{FindRep}(\ck,\eps)$. For all subsets $F \subseteq R$, we find a basic optimal solution $\bar{\lambda}^F$ of the $\textnormal{LP}(\ck,F)$ and define $C_F = \{\ell \in E_F~|~ \bar{\lambda}^F_{\ell} \geq 1\} \cup F$ as the  {\em configuration} of $F$. The configuration of $F$ is called the {\em solution } of $F$ if it forms a solution of $\ck$. Finally, our algorithm chooses among the solutions of all $F \subseteq R$ a solution $C_{F^*}$ with maximal total profit. The pseudocode of our scheme is given in Algorithm~\ref{alg:EPTAS}. %The following is the main result of this paper. 
%
\begin{theorem}
	\label{thm:EPTAS}
	Algorithm~\ref{alg:EPTAS} is an \textnormal{EPTAS} for \textnormal{BMI}.
\end{theorem}

\begin{proof}
	Let $\ck =  (E,\cI,s,p)$ be a BMI instance, $0<\eps <\frac{1}{2}$, and $A = \textsf{EPTAS}(\ck, \eps)$. By Step~\ref{step:init}, Step~\ref{step:iff} and Step~\ref{step:update} of Algorithm~\ref{alg:EPTAS} it holds that $A$ is a solution of $\ck$.  We now provide a lower bound on the profit of $A$. 
	
	Let $U$ be a solution of $\ck$ with profit $p(U) = \OPT(\ck)$. In the following, we partition a subset (with possibly empty sets in the partition) of the profitable elements in $U$ into $\eps^{-1}$ disjoint sets. Formally, for all $i \in \left[\eps^{-1}\right]$ let 
	%
	\begin{equation}
		\label{J_i}
J_i = \big\{\ell \in H \cap U~\big|~ p(\ell) \in \big[\eps^{i+1} \cdot \OPT(\ck),  \eps^{i} \cdot \OPT(\ck) \big) \big\}		
	\end{equation}
	%
 be all profitable elements in $U$ with profits in the interval $ \big[\eps^{i+1} \cdot \OPT(\ck),  \eps^{i} \cdot \OPT(\ck) \big) $. Since $J_1,\ldots, J_{\eps^{-1}}$ are $\eps^{-1}$ disjoint  subsets of elements within $U$, there is $i^* \in \left[\eps^{-1}\right]$ such that $p(J_{i^*}) \leq \eps \cdot \OPT(\ck)$ as otherwise it implies that $p(U) > \OPT(\ck)$ in contradiction. Now, define $J_0 = (H \cap U) \setminus \bigcup_{i \in [\eps^{-1}]} J_i$ as the set containing the largest profitable elements in $H \cap U$ not counted in the above subsets; in addition, let $L =  \bigcup_{k < i^*} J_k$ (including $J_0$) be the {\em most profitable} elements. %and $Q = U \setminus (L \cup J_{i^*})$ the {\em less profitable} elements. 
 	\begin{claim}
 	\label{claim:q}
 	$L \in \cI^{q(\eps)}$. 
 \end{claim}
 %Since $L \subseteq H \cap U$, by the hereditary property it holds that $L \in \cI$; in addition, since $q(\eps) = \eps^{-t-1}$ and $p(\ell) \geq \eps ^{t} \cdot \OPT ~\forall \ell \in H \cap U$, it holds that $|L| \leq q(\eps)$ or $p(L) > \OPT(\ck)$ in contradiction that $L$ is a solution of $\ck$. Hence, $L \in \cI^{q(\eps)}$; then, 
 By Claim~\ref{claim:q}, the conditions of Theorem~\ref{lem:main} are satisfied for $L$; hence, there is $Z \subseteq R$, where $R = \textsf{FindRep}(\ck,\eps)$, such that $Z \in \cI^{q(\eps)}$, $s(Z) \leq s(L)$, $|Z| = |L|$, and $p(Z) \geq (1-\eps) \cdot p(L)$.  Then, because $Z \subseteq R$, there is an iteration of Algorithm~\ref{alg:EPTAS} such that $F = Z$ in Step~\ref{step:for}. %We use the following auxiliary claim whose proof is given in Section~\ref{sec:proofs}.
	%
	\begin{claim}
		\label{claim:x}
		There is a point $\bar{x}^*$ in $\textnormal{LP}(\ck,Z)$ such that $p(Z)+\sum_{\ell \in E_Z} \bar{x}^*_{\ell} \cdot p(\ell) \geq (1-4 \eps) \OPT(\ck)$.
	\end{claim}
%
	Recall the optimal vertex solution to $\textnormal{LP}(\ck,Z)$, that is $\bar{\lambda}^Z$, constructed in Step~\ref{step:vertex} of Algorithm~\ref{alg:EPTAS} in the iteration for $F = Z$. Now, 
	%
	%
		\begin{equation*}
		\label{eq:p(x)}
		\begin{aligned}
			p(A) \geq{} & p(C(Z)) \geq  p(Z)+\sum_{\ell \in E_Z} \bar{\lambda}^Z_{\ell} \cdot p(\ell) -2\eps \cdot \OPT(\ck) \geq (1-6 \eps) \OPT(\ck)
		\end{aligned}
	\end{equation*} The first inequality is because $Z \in \cI$ and $s(Z) \leq s(L) \leq s(U) \leq 1$; it follows that $C(Z)$ is a solution of $\ck$ and $A$ is updated in Step~\ref{step:update} to be a solution of at least the same profit. The second inequality is because the LP in \eqref{LP} is in a face of dimension $1$ of the $Z$-matroid polytope $P_{\cm_Z}$; then, by Lemma~\ref{lem:integral} there are at most $2$ fractional entries in $\bar{\lambda}^Z$; in addition, the fractional entries correspond to elements in $E_Z$ with profits at most $\eps \cdot \OPT(\ck)$ by \eqref{E_F}, since for all $\ell \in E$ it holds that $p(\ell) \leq \OPT(\ck)$. The third inequality is by Claim~\ref{claim:x} and because $\bar{\lambda}^Z$ is an optimal solution to $\textnormal{LP}(\ck,Z)$. By the above and using parameter $\delta = \frac{\eps}{6}$, we have the desired approximation guarantee, where the running time of Algorithm~\ref{alg:EPTAS} is of an EPTAS algorithm by the next claim, proven in Section~\ref{sec:proofs}. \begin{claim}
	\label{lem:runningTime} For any  \textnormal{BMI} instance $\ck$ and $0<\eps <\frac{1}{2}$, Algorithm~\ref{alg:EPTAS} runs in time $O(2^{q^2(\eps)}) \cdot |\ck|^{O(1)}$. 
\end{claim}
	%(\max\{|Z|-|Q|,0\}) \eps^{i^*+1} \cdot p(B^*)  
%
\end{proof}

\comment{arg1
We construct the {\em profit classes} as the set containing the possible profits of profitable elements after the rounding (i.e., by $\bar{p}$), that is $T = \{\bar{p}(\ell)~|~\ell \in H\}$ and assume that for all $\ell \in I$ it holds that $p(\ell) \leq \OPT(\cI)$ since otherwise $\ell$ does not belong to any solution of $\mathcal{I}$.


\begin{lemma}
	\label{T}
	$|T| \leq q$. 
\end{lemma}

\begin{proof}
	
	
	Let $r^* =  \max_{\{r \in \mathbb{N}~|~ r \cdot \eps \cdot h \in T\}} r$. If $r^* >q$, it holds that there is an element$\ell \in E$ such that $$p(\ell) = r^* \cdot \eps \cdot h > q \cdot \eps \cdot  h = 2 \cdot \eps^{-t-1} \cdot \eps \cdot \eps^{t} \cdot p(B^*) = 2p(B^*)  \geq \OPT(\cm).$$ We reach a contradiction since for all $\ell \in E$ it holds that $p(\ell) \leq \OPT(\cm)$ and the claim follows. 
	
\end{proof}
}


\comment{



In the following we describe the construction of a subset of elements $S \subseteq I$ for the proof of Theorem~\ref{thm:guess}. Let $y \in T$  be a profit class. We choose up to $2q$ groups, and from each group we take up to $2q$ elements with profit $y$ for $S$. This is done greedily, where we take elements small as possible as explained next more concretely.  

We define the following order on $\cG$. Let $y \in T$ be a profit class. Let $\cG_y = \{G \in \cG~|~\exists \ell \in G \text{ s.t. } p(\ell) = y\}$. For all $G \in \cG_y$, let \begin{equation}
	f_y(G) = \min_{\ell \in G \text{ s.t. } p(\ell) = y} s(\ell).
\end{equation} In words, $f_y(G)$ is the minimal size of an element in $G$ with profit exactly $y$.  Let $|\cG_y| = n$ and let $G_1, \ldots, G_n$ be a non decreasing order of $\cG_y$ by the function $f_y$. Finally, let $q_y = \max\{2q, |\cG_y|\}$. These are the {\em representative groups} for $y$ and let $F(y) = \{G_1, \ldots, G_{q_y}\}$ be this set of groups. For each representative group $G \in F(y)$ we choose the {\em representative elements} as follows. Let $G(y) = \{\ell \in G~|~p(\ell) = y\}$ be the elements in $G$ with profit $y$. Now, let $\ell_1, \ldots, \ell_{\alpha}$ be the elements in $G(y)$ according to a non decreasing order by the element sizes (the function $s$). We define the representative elements as the set $G^i(y) =  \{\ell_1, \ldots, \ell_{\beta}\}$ where $\beta = \min\{2q, |\cG(y)|\}$ elements in the above order. 

Finally, let the $y${\em-elements} be the union of the representative elements for all representative groups of $y$:  $S_y = \bigcup_{i \in [q_y]} G^i(y)$. Then, our algorithm then computes the union of the $y$-elements for all profit classes $y \in T$. That is, $S = \bigcup_{y \in T} S_y$. The pseudocode of Algorithm \textsf{Profitable} is given in Algorithm~\ref{alg:guess}. 


\comment{arg1
	\begin{equation}
		\label{D}
		S_y = \bigcup_{i \in [q_y]} G^i(y). 
\end{equation}} 


\begin{algorithm}[h]
	\caption{$\textsf{Profitable}(\mathcal{I} = (I,\cG,s,p,m,c), \eps)$}
	\label{alg:guess}
	%Compute the instance $\mathcal{J} = (I,\cG,s,\bar{p},m,c)$. 
	
	For each $y \in T$ compute the $y$-elements $S_y$. 
	
	Return $S = \bigcup_{y \in T} S_y$. 
\end{algorithm}


\begin{lemma}
	\label{S}
	$S$ returned by Algorithm~\ref{alg:guess} satisfies $|S| \leq \exp(\eps^{-3})$.
\end{lemma}

\begin{proof}
	We use the following inequality:
	
	\begin{equation}
		\label{q3}
		\begin{aligned}
			q^3 ={} & \left(\ceil{2 \cdot \eps^{-t-1}} \right)^3 \leq \left(2 \cdot \eps^{-t-1}+1\right)^3 \leq \left(2 \cdot \eps^{-t-1}+2 \cdot \eps^{-t-1}\right)^3 \leq  \left(\eps^{-t-2}\right)^3 \\ 
			\leq{} &	\left(\eps^{-\eps^{-1}-3}\right)^3 \leq 	\left(\eps^{-2\eps^{-1}-}\right)^3 = \eps^{-6\eps^{-1}} \leq \eps^{-\eps^{-2}}   \leq \exp(\eps^{-1})^{\eps^{-2}} \leq \exp(\eps^{-3}). 
		\end{aligned}	
	\end{equation} The inequalities follow since $0<\eps<0.1$. Now, 
	
	$$|S| = \left|\bigcup_{y \in T} S_y\right| \leq \bigcup_{y \in T} \left|S_y\right| \leq |T| \cdot 2q\cdot 2q \leq 4q^3 \leq 4 \exp(\eps^{-3}) \leq \exp(\eps^{-4}).$$ The second inequality is by the definition of the $y$-elements. The third inequality is by Lemma~\ref{T}. The fourth inequality is by \eqref{q3}. 
\end{proof}

\begin{lemma}
	The running time of Algorithm~\ref{alg:guess} is $f(1/\eps) \cdot |\cI|^{O(1)}$. 
\end{lemma}

\begin{proof}
	Computing $X$ is polynomial in $ |\cI|^{O(1)}$ by \cite{fleischer2011tight}. Then, we can also compute $\cJ$ in polynomial time. As $|T|$ and $q$ are bounded by a function of $1/\eps$, we can also compute the $y$-elements for all $y \in T$ in polynomial time. 
\end{proof}

For the proof of Theorem~\ref{thm:guess}, given an optimal solution $Z$ of $\mathcal{J}$ we construct a solution as explained next. This requires some definitions. Let $A$ be a solution of $\mathcal{J}$ and let the profitable elements assigned to a bin of $A$ be $$\textsf{elements}(A) = H \cap \bigcup_{i \in [m]} A_i.$$ Moreover, let $\cG_A = \{G \in \cG~|~ G \cap \textsf{elements}(A) = \emptyset\}$ be the set of groups that do not contain a profitable elementin the solution $A$. For all $\ell \in I$, $G \in \cG$ such that $\ell \in G$, let $\textsf{group}(\ell) = G$ be the {\em group of} $\ell$. Finally, for all $y \in T$ let $S_y[A] = \{\ell \in S_y ~|~ \textsf{group}(\ell) \notin \cG_A\}$ be the elements in $S_y$ of groups disjoint to the solution $A$ and let the elementof smallest size in this set be\footnote{assume that the elements have distinct sizes, or choose arbitrarily an elementof smallest size.}

\begin{equation}
	\label{item}
	\ell_y[A] = \arg \min_{\ell \in S_y[A]} s(\ell). 
\end{equation} Furthermore, let $A_y = \textsf{elements}(A) \cap \{\ell \in I ~|~p(\ell) = y\}$ be profitable elements in $A$ with profit $y$. We do the following process. We start with an optimal solution $Z^0$ for $\mathcal{J}$. If there is $y \in T$ such that $Z^0_y \setminus S \neq \emptyset$, then let  $i \in [m]$ such that there is $\ell \in (Z^0_i \cap Z^0_y) \setminus S$; we define an {\em exchange} in $Z_i$: let $Z^1_i = (Z^0_i \setminus \{\ell\}) \cup \{\ell_y[Z^0]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^1_j = Z^0_j$; finally, let $Z^1 = (Z^1_1, \ldots, Z^1_m)$ be the solution after one iteration and let $S^1 = S \setminus \{\ell_y[Z^0]\}$.

In general, after $r$ iterations, the process finds $y \in T$ (if exists) such that $Z^r_y \setminus S^{r} \neq \emptyset$, then chooses arbitrary $i \in [m]$ such that there is $\ell \in (Z^{r}_i \cap Z^{r}_y) \setminus S^{r}$; we define an {\em exchange} in $Z^r_i$: let $Z^{r+1}_i = (Z^{r}_i \setminus \{\ell\}) \cup \{\ell_y[Z^{r}]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^{r+1}_j = Z^r_j$; finally, let $Z^{r+1} = (Z^{r+1}_1, \ldots, Z^{r+1}_m)$ be the solution after iteration $r$. The pseudocode of the process is given in Algorithm~\ref{alg:2}. 

\begin{algorithm}[h]
	\caption{$\textsf{solution}(\cJ, Z^0)$}
	\label{alg:2}
	
	Initialize $r = 0$. 
	
	
	\While{$\exists y \in T$ such that $Z^r_y \setminus S^{r} \neq \emptyset$ }{
		
		Let $i \in [m]$ such that there is $\ell \in (Z^{r}_i \cap Z^{r}_y) \setminus S^{r}$. 
		
		Let $Z^{r+1}_i = (Z^{r}_i \setminus \{\ell\}) \cup \{\ell_y[Z^{r}]\}$ and for all $j \in [m] \setminus \{i\}$ let $Z^{r+1}_j = Z^r_j$. 
		
		Let $Z^{r+1} = (Z^{r+1}_1, \ldots, Z^{r+1}_m)$
		
		Update $r \leftarrow r+1$. 
	}
	
	Return $B = Z^r$ and $A = (Z^r_1 \cap H, \ldots, Z^r_b \cap H)$. 
	
\end{algorithm}

%While there are $i \in [m]$, $\ell \in Z_i \setminus S$ such that $p(\ell) = y$, then let 

%We use the following bin structuring technique from \cite{jansen2010parameterized}. 
}


\comment{
\section{Properties of the Representative Elements}
\label{sec:lemMainProof}

In this section we prove Theorem~\ref{lem:main} mainly based on simple properties of matroids. For all $r \in [2 \cdot q(\eps)]$ let $ E_r =\left((E, \cI) \bigoplus \left\{e \in E~\bigg|~p(e) \in \left[(1+\eps)^{r-1} \cdot  \eps^{t+1} \cdot p(S^{*}), (1+\eps)^r \cdot  \eps^{t+1} \cdot p(S^{*})\right]\right\}\right)^{q(\eps)}$. %For all $y \in T$, By the following lemma, given some independent set $F$, each elementin $F$ can be replaced by an elementfrom the representative elements, with the same profit and smaller size, while resulting in an independent set.  

\begin{lemma}
	\label{lem:1}
	For all $r \in [2 \cdot q(\eps)]$, $F \in \cI^{q(\eps)}$, and $d \in F \cap \left(E_r \setminus B_r \right)$, there is $b \in B_r$ such that (i) $F-d+b \in  \cI^{q(\eps)}$ and (ii) s$\left(b\right) \leq s(d)$. 
\end{lemma}




\begin{proof}
	%Assume towards a contradiction that for all $b \in B_r$ such that $F-d+b \in  \cI^{q(\eps)}$ it holds that s$\left(b\right) > s(d)$. Observe that $|B_r| \geq 1$ because $d \in E_r$ and $B_r \subseteq E_r$; hence, by Lemma~\ref{lem:prel} there is $D \subseteq B_r, |D| = |B_r|-1$ such that $D+d \in   \cI^{q(\eps)}$. Because  $ |D| = |B_r|-1$, there is exactly one $e \in B_r \setminus D$; by the assumption, it holds that $s(e) > s(d)$ and it follows that $s(D+d) < s(B_r)$. Then, because $D+d \in   \cI^{q(\eps)}$ and $|D+d| = |B_r|$ it holds that $D+d$ is a basis of $E_r$ and  $s(D+d) < s(B_r)$ in contradiction that $B_r$ is a minimal basis of $E_r$ w.r.t. $s$.  
	
	
	
	
\comment{arg1	Let $n = |B_y|$ and for all $i \in [n]$ let $b_i$ be the $i$-th element added to $B_y$ in Algorithm \textsf{Chosen}; in addition, let $	R(i) = \{b_j~|~i \in [n], b_j < b_i\}$ be the first elements added to $B_y$ until the predecessor element to $y(b_i)$.

 Let the elementadded to $B_y$ which satisfies (i) and with minimal size be \begin{equation}
		\label{b*}
		b^* = \arg \min_{\{b \in B_y ~|~  F-d+b \in \cI\}} s(b).
	\end{equation} If there is more than one such $b^*$ choose the first such elementadded to $B_y$. We use the following variable. First, if there is no $b \in B_y$ such that $F-d+b \in \cI$ then let $R = \emptyset$; otherwise, let $R = \{b \in B_y~|~ s(b)<s(b^*)\}$ be all elements added to $B_y$ before element$b^*$. Observe that for all $b \in R$ it holds that $s(b)<s(b^*)$ since $b^*$ is the first elementadded to $B_y$ with size $s(b^*)$. Assume towards a contradiction that $s\left(b^*\right) > s(d)$. We reach in two complementary cases, as follows. }





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Define the subset of elements in $B_y$ satisfying (i) and (ii) as: 

\begin{equation}
	\label{R}
	R = \{b \in B_y~|~ F-d+b \in \cI^q, s(b) \leq s(d)\}. 
\end{equation} If $R \neq \emptyset$ the claim follows by \eqref{R}. Therefore, Assume towards a contradiction that $R = \emptyset$. Because $d \in F$, it follows that $|R|<|F|$. Then, by Property~1 of Lemma~\ref{lem:prel} there is $C \in F \setminus R, |C| = |F|-|R|$ such that $R \cup C \in \cI^q$. We use the following auxiliary claim. 

\begin{claim}
\label{dC}
$d \notin C$. 
\end{claim}
%Second, $|B| \leq |R|<|F| \leq q$ (recall that $F \in \cI^q$) and it holds that $|B| \leq q-1$. 
\begin{proof}
Assume towards a contradiction that $d \in C$; thus, since $R \cup C \in \cI^q$ and $\{d\} \subseteq C$, we get by the hereditary property that $R+d \in \cI^q$. Let $B$ be the temporary set $B_y$ right before Step~\ref{step:if} of Algorithm~\ref{alg:representative} for $y(i) = d$. Observe that $B \subseteq R$ by \eqref{R} and by the ordering of the elements in Step~\ref{order} of Algorithm~\ref{alg:representative}. Then, because $R+d \in \cI^q$ then by the hereditary property it follows that $B+d \in \cI^q$. Therefore, by Step~\ref{step:if} of Algorithm~\ref{alg:representative}, we should add $d$ to $B_y$ and it follows that $d \in B_y$ in contradiction. 
\end{proof} 	Therefore, $|R \cup C| = |F|> |F-d|$ since $d \in F$; by the exchange property of $(E,\cI^q)$, there is $b^* \in (R \cup C) \setminus (F-d)$ such that $F-d+b \in \cI^q$. Since $C \subseteq F$ and $d \notin C$ by Claim~\ref{dC}, it holds that $C \subseteq F-d$; it follows that $b^* \in R$ in contradiction that $R = \emptyset$. 
%Observe that $d \notin R$ since $d \notin B_y$. 


\end{proof}

%We split the proof into two complementary cases and in each show the existence of $b^* \in B_y$ which satisfies (i) and (ii). 
	\comment{arg1
	\begin{itemize}
		\itemIf $|R| \geq |F|$. Then, it follows that $|R| \geq |F| > |F-d|$ since $d \in F$. Therefore, by the exchange property of $(E,\cI^q)$, there is $b^* \in R \setminus (F-d)$ such that $ F-d+b^* \in \cI^q$. Hence, by \eqref{R} we have that $b^*$ satisfies the conditions of the lemma.%By the definition of $R$ we have that $s(b)<s(b^*)$ in contradiction to \eqref{b*}.
		
		\itemIf $|R| < |F|$. 
	}
		
		


	\noindent{\bf Proof of Lemma~\ref{lem:main}}:  Let $Z \in \cI^q$ such that (a) $s(Z) \leq s(G)$, (b)  for all $y \in T$ it holds that $|E_y \cap Z| = |E_y \cap G|$ and $|Z \cap S|$ is maximal among all $Z' \in \cI^q$ satisfying (a) and (b). Assume towards a contradiction that there is $a \in Z \setminus S$ and let $y = p(a)$.  Because $a \notin S$ and $B_y \subseteq S$, by Lemma~\ref{lem:1} there is $b^* \in B_y$ such that (i) $Z-a+b^* \in \cI^q$ and (ii) $s(b^*) \leq s(a)$; we define $W = Z-a+b^*$. It holds that $s(W) = s(Z)-s(a)+s(b^*) \leq s(Z)$ by (ii). In addition, for all $y' \in T -y$ it holds that $|E_{y'} \cap W| = |E_{y'} \cap G|$ and $|E_{y} \cap W| = |E_{y} \cap G|$ because $a, b^* \in E_y$ and by (b). Furthermore, $|W \cap S| > |Z \cap S|$ because $a \notin S$ and $b^* \in S$. Hence, $W$ satisfies (a), (b) and $|W \cap S| > |Z \cap S|$ which contradicts the maximality of $|Z \cap S|$. \qed



\comment{
\section{Deferred Proofs}
\label{sec:proofs}

\comment{

	\noindent{\bf Proof of Lemma~\ref{lem:J}}: 
	We use the following inequality. For any $\ell \in H$, by \eqref{eq:max} there is $r \in \mathbb{N}$ such that $\bar{p}(\ell) = r \cdot \eps \cdot h$ and $p(\ell) < (r+1) \cdot \eps \cdot h$; therefore,  		\begin{equation}
			\label{claim:1}
			p(\ell)-\bar{p}(\ell) \leq (r+1) \cdot \eps \cdot h- r \cdot \eps \cdot h =  \eps \cdot h \leq \eps \cdot p(\ell).
		\end{equation} The first inequality is by \eqref{eq:max}. The second inequality is because $\ell \in H$. Now, 
%	\end{proof} 


	
	$$\bar{p}(A) = \sum_{\ell \in A} \bar{p}(\ell) \geq \sum_{\ell \in A} (1-\eps) \cdot p(\ell) = (1-\eps) \sum_{\ell \in A} p(\ell) = (1-\eps) \cdot p(A).$$ The inequality follows for all $\ell \in E \setminus H$ since $\bar{p}(\ell) = p(\ell) \geq (1-\eps) p(\ell)$; furthermore, for all $\ell \in H$ the inequality follows by \eqref{claim:1}.\qed


}



	\noindent{\bf Proof of Claim~\ref{claim:q}}: 
	%
	Since $L \subseteq H \cap U$, by the hereditary property it holds that $L \in \cI$. Thus, to show that $L \in \cI^{q(\eps)}$, we show that $|L| \leq q(\eps)$. Assume towards a contradiction that $|L| > q(\eps)$. Therefore, %in addition, since $q(\eps) = \eps^{-t-1}$ and $p(\ell) \geq \eps ^{t} \cdot \OPT ~\forall \ell \in H \cap U$, it holds that $|L| \leq q(\eps)$ or $p(L) > \OPT(\ck)$ in contradiction that $L$ is a solution of $\ck$. Hence, $L \in \cI^{q(\eps)}$
	%
	\begin{equation}
		\label{contradiction1}
		\begin{aligned}
			p(U) ={} & \sum_{\ell \in U} p(\ell) \geq  \sum_{\ell \in H \cap U} p(\ell) \geq \sum_{\ell \in L}  \eps^{t} \cdot \OPT(\ck)  = \eps^{t} \cdot \OPT(\ck) \cdot |L| \\ >{} & \eps^{t} \cdot \OPT(\ck) \cdot q(\eps) =\eps^{-1} \cdot \OPT(\ck) >  \OPT(\ck). 
		\end{aligned}
	\end{equation} The second inequality is because for all $\ell \in H$ it holds that $p(\ell) \geq  \eps^{t} \cdot \OPT(\ck)$. The third inequality is by the assumption that $q(\eps) < |L|$. By \eqref{contradiction1} we reach a contradiction since $p(U) =  \OPT(\ck)$.  \qed
	%We split the proof into the two parts (i) and (ii). 
\comment{
\begin{itemize}
	\item(i). 	Assume towards a contradiction that there is a solution $A$ of $\cm$ such that $q < |H \cap A|$. Therefore, 
	
	
	
	\begin{equation}
		\label{contradiction1}
		\begin{aligned}
			p(A) ={} & \sum_{\ell \in A} p(\ell) \geq  \sum_{\ell \in H \cap A} p(\ell) \geq \sum_{\ell \in H \cap A} h   = h \cdot |H \cap A| > h \cdot q = \eps^{t} \cdot p\left(B^*\right) \cdot 2 \eps^{-t-1} \\ ={} & 2 \cdot p\left(B^*\right)  \eps^{-1} \geq \OPT(\cm) \cdot \eps^{-1}  >   \OPT(\cm). 
		\end{aligned}
	\end{equation} The second inequality is because for all $\ell \in H$ it holds that $p(\ell) \geq h$. The third inequality is by the assumption that $q < |H \cap A|$. the fourth inequality is because $B^*$ is a $2$-approximation for $\cm$. By \eqref{contradiction1} we reach a contradiction that $A$ is a solution of $\cm$ with profit strictly larger than $\OPT(\cm)$. 
	
	\item(ii). 	Let $r^* =  \max_{\{r \in \mathbb{N}~|~ r \cdot \eps \cdot h \in T\}} r$. If $r^* >q$, it holds that there is an element$\ell \in E$ such that $$p(\ell) = r^* \cdot \eps \cdot h > q \cdot \eps \cdot  h = 2 \cdot \eps^{-t-1} \cdot \eps \cdot \eps^{t} \cdot p(B^*) = 2p(B^*)  \geq \OPT(\cm).$$ We reach a contradiction since $A = \{\ell\}$ is a solution with $p(A) > \OPT(\cm)$. By the above, $|T| \leq |\{r \in[q]\}| = q.$ \qed
\end{itemize}
}


	
		\noindent{\bf Proof of Claim~\ref{claim:x}}: 
		Let $Q = U \setminus (L \cup J_{i^*})$. Because $U \in \cI$ and $Q \subseteq U$, by the hereditary property it follows that $Q \in \cI$. We define a point in $\textnormal{LP}(\ck,Z)$ whose definition is relied on the following subset of elements. First, if $|Z| > |Q|$ then define $C = \emptyset$. Otherwise, $|Q| \geq |Z|$; then, by Lemma~\ref{lem:prel} there is $C' \subseteq Q \setminus Z, |C'|  = |Q| - |Z|$ such that $Z \cup C' \in \cI$; in this case, define $C = C'$. Now, define $\bar{x}^* \in \{0,1\}^{E_Z}$ such that for all $\ell \in C$ define $\bar{x}^*_{\ell} = 1$ and for all $\ell \in E_Z \setminus C$ define $\bar{x}^*_{\ell} = 0$. 
		
		It is shown below that $\bar{x}^*$ satisfies the conditions of $\textnormal{LP}(\ck,Z)$. Because $Z \cup C \in \cI$, it follows by the definition of the matroid polytope that $\bar{x}^* \in P_{\cm_Z}$, the $Z$-matroid polytope. In addition, $$\sum_{\ell \in E_Z} \bar{x}^*_{\ell} \cdot s(\ell) = \sum_{\ell \in C} s(\ell) \leq \sum_{\ell \in Q} s(\ell) = s(Q) \leq 1-s(U \setminus Q) \leq 1-s(L) \leq 1-s(Z).$$ The second inequality is because $U$ is a solution of $\ck$. The last inequality is by Lemma~\ref{lem:main}. By the above and by \eqref{LP}, it holds that $\bar{x}^*$ satisfies the conditions of $\textnormal{LP}(\ck,Z)$. To conclude the proof, we use the following inequalities. If $L \neq \emptyset$ the following holds:
		%
		\begin{equation}
			\label{eq:11}
			\begin{aligned}
				\eps \cdot p(Z)-p(Q \setminus C) \geq{} & 	\eps \cdot p(Z)-|Q \setminus C| \cdot \max_{\ell \in Q \setminus C} p(\ell) \geq \eps \cdot p(Z)- |Z| \cdot \eps \cdot  \min_{\ell \in L} p(\ell) \\ \geq{} & \eps \cdot p(Z)- |Z| \cdot   \frac{\eps \cdot \min_{\ell \in Z} p(\ell)}{(1-\eps)} \geq \eps \cdot p(Z)-2\eps \cdot p(Z) \geq -\eps \cdot \OPT(\ck).
			\end{aligned}
		\end{equation} The second inequality is because $C \subseteq Q \setminus Z$, $|C|  = |Q| - |Z|$ or $C = \emptyset$ if $|Z| > |Q|$ and it follows that $|Q \setminus C| \leq |Z|$; in addition, by \eqref{J_i} and the definition of $L,Q$ it holds that all elements in $Q \setminus C$ are of profits at most $\eps \cdot \min_{\ell \in L} p(\ell)$ for $L \neq \emptyset$. The third inequality is by Lemma~\ref{lem:main}. The fourth inequality is because $0<\eps <\frac{1}{2}$. The last inequality is because $p(Z) \leq \OPT(\ck)$, since $Z$ is a solution of $\ck$ because $L$ is a solution of $\ck$ and by Lemma~\ref{lem:main}. Furthermore, 
		%
		\begin{equation}
			\label{eq:p(x)2}
			\begin{aligned}
				p(Z)+p(Q) \geq{} & (1-\eps) \cdot p(L)+ p(Q) \geq  (1-\eps) \left( p(L)+p(Q)\right) =  (1-\eps)  p(U \setminus J_{i^*}) \\ \geq{} & (1-\eps) (1-\eps)\OPT(\ck) \geq (1-2\eps)  \OPT(\ck). 
			\end{aligned}
		\end{equation} The first inequality is by Lemma~\ref{lem:main}. The third inequality is because $p(J_{i^*}) \leq \eps \cdot \OPT(\ck)$. Therefore,%The first equality is because $Z,L \subseteq H$ and for all $y \in T$ it holds that $|Z \cap E_y| = |E_y \cap L|$. The second inequality is by Lemma~\ref{lem:J}. Therefore,
		%
		\begin{equation*}
			\label{eq:p(x)}
			\begin{aligned}
				p(Z)+\sum_{\ell \in E_Z} \bar{x}^*_{\ell} \cdot p(\ell) ={} & p(Z)+\sum_{\ell \in C} p(\ell) = p(Z)+p(C) = p(Z)+p(Q) - p(Q \setminus C) \\ \geq{} & (1-\eps) (p(Z)+p(Q))+\eps \cdot p(Z)-p(Q \setminus C)  \geq (1-4\eps) \OPT(\ck).
			\end{aligned}
		\end{equation*} The last inequality is by \eqref{eq:11} and \eqref{eq:p(x)2}.  Hence, $\bar{x}^*$ satisfies the conditions of the claim. \qed
	
	
		\noindent{\bf Proof of Claim~\ref{lem:runningTime}}: 
	}
}
